Adaptive Model Predictive Control of Wheeled Mobile Robots

In this paper, a control algorithm for guiding a two wheeled mobile robot with unknown inertia to a desired point and orientation using an Adaptive Model Predictive Control (AMPC) framework is presented. The two wheeled mobile robot is modeled as a knife edge or a skate with nonholonomic kinematic constraints and the dynamical equations are derived using the Lagrangian approach. The inputs at every time instant are obtained from Model Predictive Control (MPC) with a set of nominal parameters which are updated using a recursive least squares algorithm. The efficacy of the algorithm is demonstrated through numerical simulations at the end of the paper.

==> 3MPC.tex <==
\section{MPC Algorithm}
To begin, we built a constrained finite time optimal control function in Python using the solver “ipopt” from the IPOPT optimization package.  This constrained finite time optimal control (CFTOC)  function incorporated both state constraints based on system dynamics and input constraints based on the predicted mechanical limits of the robot system. In addition, it was designed to optimize the robot trajectory so that it would arrive at a specific set of desired terminal states. Actual system parameters were given to the function, and a batch approach was used to calculate an optimal set of states and inputs. The results, with all system parameters known, can be seen in figures seven through nine in the Appendix.

This CTFOC function is feasible since Python was able to calculate an optimal series of states and inputs.

To further optimize, the CTFOC function was implemented in a larger MPC function, so that the optimal states and inputs would be recalculated at each time step. Graphs and simulations show the accuracy of the MPC control.  However, determining the persistent feasibility of this MPC simulation is difficult to prove since the problem is nonlinear. 
	
Initially the system parameters such as mass, moment of inertia and damping, were assumed to be constant in these simulations. However, to increase the usefulness and relevance of the control algorithm, it was instead assumed that these parameters were unknown, and a new function was implemented to help the controller adapt. See section IV. 

